Deep Reparametrization of Multi-Frame Super-Resolution and Denoising

We propose a deep reparametrization of the maximum a posteriori formulation commonly employed in multi-frame image restoration tasks. Our approach is derived by introducing a learned error metric and a latent representation of the target image, which transforms the MAP objective to a deep feature space. The deep reparametrization allows us to directly model the image formation process in the latent space, and to integrate learned image priors into the prediction. Our approach thereby leverages the advantages of deep learning, while also benefiting from the principled multi-frame fusion provided by the classical MAP formulation. We validate our approach through comprehensive experiments on burst denoising and burst super-resolution datasets. Our approach sets a new state-of-the-art for both tasks, demonstrating the generality and effectiveness of the proposed formulation.

==> related_work_looong.tex <==
\section{Related Work}
\parsection{Multi-Frame Super-Resolution} MFSR is a well-studied problem and numerous approaches have been proposed for the same in literature. Tsai and Huang~\cite{Tsai1984MultiframeIR} were the first to propose a frequency-domain based solution for MFSR. Peleg~\etal~\cite{Peleg1987ImprovingIR} proposed an iterative approach based on an image formation model. Here, an initial guess of the SR image is first obtained and then refined by minimizing the reconstruction error. Irani and Peleg~\cite{Irani1991ImprovingRB} later employed the back-projection algorithm used in Computer Aided Tomography to minimize the reconstruction error. Several works~\cite{Bascle1996MotionDA,Schultz1996ExtractionOH,Elad1997RestorationOA,Hardie1998HighResolutionIR} extended the objective in~\cite{Irani1991ImprovingRB} with a regularization term to obtain a maximum a posteriori (MAP) estimate of the HR image. The resulting optimization problem was minimized using gradient-based methods, \eg conjugate-gradients~\cite{Bascle1996MotionDA,Hardie1998HighResolutionIR}. In order to be robust to outliers,~\cite{Zomet2001RobustS} proposed a median estimator for gradients. Alternatively, Farsiu~\etal~\cite{Farsiu2004MultiframeDA} proposed using $L_1$ norm for calculating the reconstruction error and introduced a bilateral prior to further promote robustness. He and Kondi~\cite{He2006AnIS} introduced a weighted reconstruction error to generalize to input images with varying noise levels. \cite{Gotoh2004DirectSA,Farsiu2004MultiframeDA} extend to MAP formulation to perform joint multi-frame demosaicking and super-resolution. 

The approaches discussed above assume that the image formation model as well as the motion between input frames is known, or reliably estimated. Several works address this limitation by jointly estimating the motion~\cite{He2007ANL,Zhang2012CommutabilityOB,Pickup2007OvercomingRU}, and/or image formation model parameters~\cite{Khler2016RobustMS,Zhang2012CommutabilityOB,Faramarzi2013UnifiedBM} together with the HR image. Another approach~\cite{Pickup2007OvercomingRU,Tipping2002BayesianIS,Pickup2009BayesianMF} is to marginalize over the unknown parameters in a Bayesian formulation. Alternatively, a number of approaches directly predict the HR image without simulating the image formation process. Chiang and Boult~\cite{Chiang2000EfficientSV} upsample and warp the input images to a common reference. The warped images are then added together and deblurred to obtain the HR estimate. Farsiu~\cite{Farsiu2003RobustSA} extend this approach with a robust regularization term. Takeda~\etal~\cite{Takeda2006RobustKR,Takeda2007KernelRF} proposed a kernel regression based approach for super-resolution. A non-local kernel regression method was later introduced by Zhang~\etal~\cite{Zhang2010NonLocalKR} for image and video restoration tasks. Recently, Wronski~\etal~\cite{Wronski2019HandheldMS} used the kernel regression technique to robustly merge images captured from a hand held camera to perform joint demosaicking and super-resolution. A few deep learning based solutions have been also proposed recently for the MFSR problem. Deudon~\etal~\cite{Deudon2020HighResnetRF} recursively fuses pairs of input images to generate the HR output, while Molini~\etal~\cite{Molini2020DeepSUMDN} use 3D convolution for fusion. Kawulok~\etal~\cite{Kawulok2019DeepLF} use a shift and add method similar to~\cite{Farsiu2003RobustSA} while using a deep network to upsample the input images. The aforementioned approaches~\cite{Deudon2020HighResnetRF,Molini2020DeepSUMDN,Kawulok2019DeepLF} are mainly focused on the remote sensing applications. In contrast, Bhat~\etal~\cite{Bhat2021DeepBS} tackle the problem of hand held burst super-resolution. Their approach explicitly aligns input images using optical flow and employs an attention-based approach for information fusion. Haris~\etal~\cite{Haris2019RecurrentBN} propose a recurrent back-projection network for the related task video super-resolution, inspired by the back-projection algorithm~\cite{Irani1991ImprovingRB}.
% Kernel regression, 


%%%%%%%%%%%%%%%%% Recon based %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% An Image Super-Resolution Algorithm for Different Error Levels Per Frame
%Hardie~\etal~\cite{Hardie1998HighResolutionIR} additionally included a regularization term in the objective, in addition to the reconstruction error, to obtain a MAP estimate of the HR image. The objective is minimized using either gradient descent or conjugate-gradient algorithm. In order to be robust to outliers,~\cite{Zomet2001RobustS} proposed a median estimator for gradients. Alternatively, Farsiu~\etal~\cite{Farsiu2004MultiframeDA} proposed using $L_1$ norm for calculating the reconstruction error and introduced a bilateral prior to further promote robustness.   

% R. Tsai and T. Huang. Multiframe image restoration and registration - fourier domain approach for MFSR
% Peleg and Irani, iterative backprojection
% R. Hardie, K. Barnard, John G. Bognar, E. Armstrong, and E. Watson. High-resolution image reconstruction from a sequence of rotated and translated frames and its application to - better observation model, regularization - 1998
% Fast and Robust Multiframe Super Resolution 2004
% Robust Super-Resolution* -- 2001


%Restoration of a single super-resolution image from several blurred, noisy, and under-sampled measured images 1997


% Motion Deblurring and Super-resolution from an Image Sequence - 2005


% Sina Farsiu, Michael Elad, and P. Milanfar. Multiframe demosaicing and super-resolution from undersampled color images. - demosaicking and SR - 2004

% A multi-frame image super-resolution method
% Bayesian Methods For Image Super-Resolution

% Bayesian combination of sparse and non-sparse priors in imagesuper resolution

% AN ADAPTIVE L1-L2 HYBRID ERROR MODEL TO SUPER-RESOLUTION

% A Fast Super-Resolution Reconstruction Algorithm for Pure Translational Motion and Common Space-Invariant Blur - fast method for only translation warps, white noise


% Robust Multiframe Super-Resolution Employing Iteratively Re-Weighted Minimization



%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Direct %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Efficient super-resolution via image warping

%Robust Kernel Regression for Restoration and Reconstruction of Images from Sparse Noisy Data
%Kernel Regression for Image Processing and Reconstruction


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\parsection{Multi-Frame Denoising} Note that the MFSR approaches discussed previously also perform denoising by leveraging information from multiple images. A number of specialized multi-frame denoising approaches have also been proposed in literature. Tico~\cite{Tico2008MultiframeID} performs block matching both within an image, as well as across the input images to perform denoising. \cite{Dabov2007VideoDB,Maggioni2011VideoDU,Maggioni2012VideoDD} extend the popular image denoising algorithm BM3D~\cite{Dabov2007ImageDB} to video. Buades~\etal~\cite{Buades2009ANO} estimate the noise level from the aligned images, and use a combination of pixel-wise mean and BM3D to denoise. Liu~\etal~\cite{Liu2014FastBI} introduced homography flow for fast alignment of input images and a robust fusion approach to handle scene motion. Hasinoff~\etal~\cite{Hasinoff2016BurstPF} used a hybrid 2D/3D Wiener filter to denoise and merge burst images for HDR and low-light photography applications. 
Recent years has also seen the introduction of deep learning based approaches for MF denoising. Godard~\etal~\cite{Godard2018DeepBD} extend a single frame denoising network for multiple frames using a recurrent neural network. Mildenhall~\etal~\cite{Mildenhall2018BurstDW} employed kernel prediction network (KPN) to obtain per-pixel kernels which are then used to merge the input images. The KPN approach was then extended by~\cite{Marinc2019MultiKernelPN} to predict multiple kernel of different sizes, while~\cite{Xia2020BasisPN} introduced basis prediction networks to enable the use of larger kernels. %\GB{include flexisp}

%  Multi-frame image denoising and stabilization.
% Video denoising, deblocking, and enhancement through separable 4-d nonlocal spatiotemporal transforms
%A NOTE ON MULTI-IMAGE DENOISING
% Multiple view image denoising
% MULTIFRAME RAW-DATA DENOISING BASED ON BLOCK-MATCHING AND 3-D FILTERING FOR LOW-LIGHT IMAGING AND STABILIZATION
% Fast Burst Images Denoising

%Deep Burst Denoising
%Burst photography for high dynamic range and low-light imaging on mobile cameras
% handheld photography in low light
% Burst Denoising with Kernel Prediction Networks
% BPN
% MULTI-KERNEL PREDICTION NETWORKS FOR DENOISING OF BURST IMAGES
%Ehret_Joint_Demosaicking_and_Denoising_by_Fine-Tuning_of_Bursts_of_Raw_ICCV_2019_paper


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\parsection{Deep Optimization-based image restoration} A number of deep learning based approaches~\cite{Zhang2017LearningDC,Kokkinos2018DeepID,Kokkinos2019IterativeRC,Zhang2020DeepUN} have also posed image restoration tasks as an explicit optimization problem. Plug-and-Play Priors ($P^3$)~\cite{Venkatakrishnan2013PlugandPlayPF} and Regularization by Denoising (RED)~\cite{Reehorst2019RegularizationBD} approaches provide a general framework for utilizing standard denoising methods as regularizers in optimization-based image restoration methods. Brifman~\etal~\cite{Brifman2019UnifiedSA} utilized these techniques to propose a unified single-image and video super-resolution approach. Zhang~\etal~\cite{Zhang2017LearningDC} used the half quadratic splitting method to plug a deep neural-network based denoiser prior into model-based optimization methods. In a similar spirit, Kokkinos~\etal~\cite{Kokkinos2018DeepID} proposed a joint denoising and demosaicking approach, with the key difference that the denoiser as well as the optimization hyper-parameters are jointly trained. The idea of learning the regularizer as a neural network was also employed for burst photography applications in~\cite{Kokkinos2019IterativeRC} using a proximal gradient descent based method. These prior works mainly focus on learning the regularizer, while assuming that the data term (image formation process) is known and simple. Furthermore, the reconstruction error computation, as well as the error minimization are restricted to be in the image space. In contrast, our deep reparametrization approach allows jointly learning the imaging process as well as the priors, without restricting the image formation model to be simple or linear.   

%\MD{also say that optimization and error metric is in image space?}

%Plug-and-Play Priors for Model Based Reconstruction
% The Little Engine that Could Regularization by Denoising (RED)
% Trainable Nonlinear Reaction Diffusion: A Flexible Framework for Fast and Effective Image Restoration
%Plug-and-Play ADMM for Image Restoration: Fixed Point Convergence and Applications


% Deep Image Demosaicking using a Cascade of Convolutional Residual Denoising Networks
%Iterative Residual CNNs for Burst Photography Applications 
% Deep Unfolding Network for Image Super-Resolution


% Non-local Color Image Denoising with Convolutional Neural Networks
%Unified Single-Image and Video Super-Resolution via Denoising Algorithms




% Deep Back-Projection Networks For Super-Resolution  --- iterative
% Recurrent Back-Projection Network for Video Super-Resolution -- iterative



%FlexISP: A flexible camera image processing framework -- not deep
% ProxImaL: Efficient Image Optimization using Proximal Algorithms (RW on Optimization for Image Processing) -- not deep

==> tables/kpn_grayscale_ablation.tex <==
\begin{tabular}{lcccc}
\toprule
&Gain $\propto$ 1&Gain $\propto$ 2&Gain $\propto$ 4&Gain $\propto$ 8\\\midrule
Ours&   39.37    &     36.51     &   33.38    &    29.69\\
No encoder&   39.20    &     36.42    &   33.38    &   29.25 \\
No decoder &    38.78  &  35.88 &  32.69   & 27.42 \\
No certainty &  39.17 &  36.34 & 33.24 & 29.43 \\
No enc + no certainty &  39.05 &  36.34 &  33.13 & 23.44 \\
No dec + no certainty &    37.83  &  35.17 & 32.22 & 28.62 \\
No dec + no enc &   38.33     &  35.33   &  31.79   & 26.57\\
No dec + no enc + no wp &   33.35     &  30.41   &  26.50   & 21.98\\

\bottomrule
\end{tabular}
